On the understanding of pulsations in the atmosphere of roAp stars: phase diversity and false nodes

Studies based on high-resolution spectroscopic data of rapidly oscillating Ap stars show a surprising diversity of pulsation behavior in the atmospheric layers, pointing, in particular, to the co-existence of running and standing waves. The correct interpretation of these data requires a careful modelling of pulsations in these magnetic stars. In light of this, in this work we present a theoretical analysis of pulsations in roAp stars, taking into account the direct influence of the magnetic field. We derive approximate analytical solutions for the displacement components parallel and perpendicular to the direction of the magnetic field, that are appropriate to the outermost layer. From these, we determine the expression for the theoretical radial velocity for an observer at a general position, and compute the corresponding pulsation amplitude and phase as function of height in the atmosphere. We show that the integral for the radial velocity has contributions from three different types of wave solutions, namely, running waves, evanescent waves, and standing waves of nearly constant amplitude. We then consider a number of case studies to illustrate the origin of the different pulsational behaviour that is found in the observations. Concerning pulsation amplitude, we find that it generally increases with atmospheric height. Pulsation phase, however, shows a diversity of behaviours, including phases that are constant, increasing, or decreasing with atmospheric height. Finally, we show that there are situations in which the pulsation amplitude goes through a zero, accompanied by a phase jumps of $\pi$, and argue that such behaviour does not correspond to a pulsation node in the outermost layers of the star, but rather to a visual effect, resulting from the observers inability to resolve the stellar surface.

==> app-A.tex <==
APPENDIX A: ORDER OF MAGNITUDE ANALYSIS
\label{app-A}

\vspace{0.3cm}
\underline{\textbf{Slow Acoustic Component}}
\vspace{0.3cm}

To derive eqs~(\ref{eq: 2.26}) and (\ref{eq: 2.25}), we have considered the order of magnitude of each term in eqs~(\ref{eq: 2.18}) and (\ref{eq: 2.19}), after separating the time and the slow and fast components of the displacement. For that we will take as a reference the solution that we would obtain in the absence of the magnetic field. The latter is of the type,

\begin{equation}
\label{eq: 2.22b}
{\xi}_{s}=\frac{A}{p^{1/2}}e^{-ikz}+\frac{B}{p^{1/2}}e^{ikz},
\end{equation}
with $A$ and $B$ being constant amplitudes and, 

\begin{equation}
\label{eq: 2.22b}
k^2=\frac{\omega^2-\omega^2_c}{c^2},
\end{equation}
where $\omega^2_c$ is the acoustic cutoff frequency defined to be $\omega_c=c/(2H)$ and $c^2={\gamma p_0}/{\rho_0}$ is the sound speed in an isothermal atmosphere \citet{1993afd..conf..399G}. In the above, $A=0$ if $\omega<\omega_c$ and $B=0$ if $\omega>\omega_c$. 

We may expect that the solution for the slow acoustic component of the displacement will vary on a scale similar to the solution in the absence of the magnetic field. Based on this assumption and considering first the case in which $B_x \approx B_z$, we can study the order of magnitude of the terms in equation (\ref{eq:2.19}). For that we use $O$ to denominate the order of magnitude, and $T_i$ to denominate the $ith$ term in the equation, with $i$ increasing from the left to the right. We start by noting that the non-magnetic solution varies typically in a scale of $H$, i.e., $O(\frac{d {\xi}_{si}}{d z})\approx H^{-1}{\xi}_{si}$. For frequencies not too far from $\omega_c$, as those seen in roAp stars, this means that $O(\frac{d {\xi}_{si}}{d z})\approx O((\omega/c) {\xi}_{si}) = O(\omega\sqrt{\rho_0/(\gamma p_0)}{\xi}_{si})$. 

%we find $O(T_1)$ is never smaller than $O((\frac{d p}{pdz} a)^2 \xi_{\bot s}))$ where $a$ is typically $1/2$. In practice $O(T_1)=max[O((\frac{dp}{pdz} a)^2\xi_{\bot s}));\frac{\omega^2 \rho_0 \left|\bm{B}_0\right|^2}{\gamma p_0 B_z^2} \xi_{\bot s}]$. 

Having this in mind we find that for equation (\ref{eq: 2.22}) the order of magnitude of the terms is as follows,

\begin{eqnarray}
O(T_1)\approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right), 
\end{eqnarray}

\begin{eqnarray}
O(T_2)\approx 0\left(\tilde{\beta}\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right), 
\end{eqnarray}

In the magnetically dominated region, $\tilde{\beta}<<1$ and, consequently, $O(T_1)>>O(T_2)$. Thus, equation (\ref{eq: 2.19}) leads, after separating the time and considering the slow component of the displacement, approximately to equation (\ref{eq: 2.23}). Looking at the latter we can conclude, under the assumptions previously made, that
\begin{equation}
\label{eq: 2.23ca}
{\xi}_{\bot s} \approx O(\tilde{\beta}{\xi}_{||s}).
\end{equation}
Therefore, we find that 
\begin{equation}
{\xi}_{\bot s}<<{\xi}_{|| s}\nonumber,
\end{equation}
which was to be expected, since in a magnetically dominated region the slow displacement is almost acoustic and, hence, takes place essentially along the magnetic field lines. 

Combining eq.~(\ref{eq: 2.23}) with eq.~(\ref{eq: 2.18}), and re-organizing the terms, we find, after separating the time and considering the slow component alone,
\begin{equation}
\label{eq: 2.34_tese}
\frac{d^2 {\xi}_{|| s} }{d z^2}+\frac{d p_0}{p_0 d z}\frac{d {\xi}_{|| s}}{d z}+\frac{\omega^2 \rho_0}{\gamma p_0}\frac{\left|\bm{B}_0\right|^2}{B_z^2}{\xi}_{||s}=-\frac{d p_0}{p_0 d z}\frac{B_x}{B_z}\frac{d {\xi}_{\bot s}}{d z}.
\end{equation}  


Next we determine the order of magnitude of the terms in eq.~(\ref{eq: 2.34_tese}). Also here we start by considering the case of $B_x\approx B_z$. Taking into account equation (\ref{eq: 2.23ca}) we can show that $O(T_3)$ and $O(T_4)$ in eq.~(\ref{eq: 2.34_tese}) are as follows,

\begin{eqnarray}
O(T_3) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\xi_{||s}\right),\nonumber
\end{eqnarray}



\begin{eqnarray}
O(T_4) \approx O\left(\frac{1}{p_0}\frac{dp_0}{dz}\sqrt{\frac{\omega^2 \rho_0}{\gamma p_0}}\tilde{\beta}\xi_{|| s}\right) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\tilde{\beta}\xi_{||s}\right).\nonumber
\end{eqnarray}
Thus, eq.~(\ref{eq: 2.34_tese}) can be written as equation (\ref{eq: 2.26}).


The order of magnitude analysis presented above assumed that $B_x\approx B_z$. However, using the solution for $\xi_{||s}$ found in this way (cf.\ eq.~(\ref{eq: 2.30c}), and returning to equations (\ref{eq: 2.18}) and (\ref{eq: 2.19}), we can show that this solution is also appropriate in the cases of $B_x$ tending to zero and $B_z$ tending to zero. The former is equivalent to considering the case in the absence of the magnetic field, so it is necessarily in accordance with the analysis made previously. Let us now consider the case of $B_z$ tending to zero. In this case the last term on the right hand side of equation (\ref{eq: 2.29}) dominates and, therefore, $k^2_{||}\approx \frac{\omega^2 \rho_0\left|\bm{B}_0\right|^2}{\gamma p_0 B_z^2}\right$. Going back to the analysis of the order of magnitude, in equation (\ref{eq: 2.19}) we have,   
\begin{eqnarray}
O(T_1)\approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\frac{|\bm{B}_0|^2}{B^2_z}{\xi}_{\bot s}\right), 
\end{eqnarray}
\begin{eqnarray}
O(T_2)\approx O\left(\tilde{\beta}\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right). 
\end{eqnarray}
Thus, we can conclude, as in the previous case, that $O(T_1)$ is always much larger than $O(T_2)$, leading back to equation(\ref{eq: 2.25}).
Moreover, from the latter we can conclude that in this case,
\begin{equation}
\label{eq: 2.23c}
{\xi}_{\bot s} \approx O\left(\tilde{\beta}\frac{B_x B_z}{|\bm{B}_0|^2}{\xi}_{||s}\right).
\end{equation}
Therefore, we find, as before,
\begin{equation}
{\xi}_{\bot s}<<{\xi}_{|| s}\nonumber.
\end{equation}


Let us now compare $O(T_3)$ with $O(T_4)$ in equation (\ref{eq: 2.34_tese}) when $B_z$ tends to zero,
\begin{eqnarray}
O(T_3) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\frac{|\bm{B}_0|^2}{B^2_z}\xi_{||s}\right),\nonumber
\end{eqnarray}
\begin{eqnarray}
O(T_4) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\tilde{\beta}\frac{B_x^2}{|B_0|^2}\xi_{||s}\right)\nonumber. 
\end{eqnarray}
Therefore, also in this case, $O(T_3)$ is larger than $O(T_4)$, and we can neglect the fourth term in equation (\ref{eq: 2.34_tese}), which leads us back to equation (\ref{eq: 2.26}).
So, we may conclude that the approximate solution expressed by equation (\ref{eq: 2.30c}), derived when considering $B_x \approx B_z$, is in fact an approximate solution for $\xi_{||s}$ in the more general case, since the terms that were neglected in the first case remain small, for this solution, when the condition $B_x \approx B_z$ is no longer satisfied. 

\vspace{0.3cm}

\underline{\textbf{Fast Magnetic Component}}

\vspace{0.3cm}

To derive eqs~(\ref{eq: 2.35}) and (\ref{eq: 2.37}) we again consider eq.(\ref{eq: 2.18}), after separating the time and the fast and slow components of the displacement. For that we shall keep in mind the condition $({\bar{\xi}}_{si})^{-1} d{\bar{\xi}}_{si}/dz >> ({\bar{\xi}}_{fi})^{-1} d{\bar{\xi}}_{fi}/dz$ that was used to distinguish the above mentioned components. Since $O(({\xi}_{si})^{-1} d{{\xi}}_{si}/dz) \approx O(\omega\sqrt{\rho_0/\gamma p_0})$, for equation (\ref{eq: 2.18}) we find,
\begin{eqnarray}
O(T_1) < < O(T_5), \nonumber
\end{eqnarray}
\begin{eqnarray}
O(T_3) < < O(T_5). \nonumber
\end{eqnarray}
Thus, equation (\ref{eq: 2.18}) leads, for the fast component of the displacement, approximately to equation (\ref{eq: 2.35}). In addition, comparing the terms in the latter equation we find that, in all cases, the fast component of the displacement perpendicular to the magnetic field is much larger than the fast component of the displacement parallel to the magnetic field, i.e.,

\begin{eqnarray}
\xi_{\bot f}>>\xi_{|| f}\nonumber.
\end{eqnarray}

Therefore we can say that the fast displacement is almost perpendicular to the direction of the magnetic field. This is not surprising, since in the magnetically dominated region this component of the displacement is expected to be essentially a magnetic wave, only slightly modified by the gas pressure.

Finally, neglecting $\xi_{|| f}$, when compared to $\xi_{\bot f}$, we find that eq.~\ref{eq: 2.19} leads, for the fast component, to eq.~\ref{eq: 2.37}.


==> app-A0.tex <==
APPENDIX A: ORDER OF MAGNITUDE ANALYSIS
\label{app-A}

\vspace{0.3cm}
\underline{\textbf{Slow Acoustic Component}}
\vspace{0.3cm}

In order to investigate if it is possible to simplify the equations for the slow acoustic component of the displacement we have considered the order of magnitude of each term in the equations (\ref{eq: 2.21})-(\ref{eq: 2.22}). For that we will take as a reference the solution that we would obtain in the absence of the magnetic field. The latter is of the type,

\begin{equation}
\label{eq: 2.22b}
{\xi}_{||s}=\frac{A}{p^{1/2}}e^{-ikz}+\frac{B}{p^{1/2}}e^{ikz},
\end{equation}

with $A$ and $B$ being constant amplitudes and, 

\begin{equation}
%\label{eq: 2.22b}
k^2=\frac{\omega^2-\omega^2_c}{c^2},
\end{equation}

where $\omega^2_c$ is the acoustic cutoff frequency defined to be $\omega_c=c/(2H)$ and $c^2={\gamma p_0}/{\rho_0}$ is the sound speed in an isothermal atmosphere \citet{1993afd..conf..399G}. In the above, $A=0$ if $\omega<\omega_c$ and $B=0$ if $\omega>\omega_c$. 

We may expect that the solution for the slow acoustic component of the displacement, that will result from equations (\ref{eq: 2.21})-(\ref{eq: 2.22}), will vary on a scale similar to the solution in the absence of the magnetic field. Based on this assumption and considering the case in which $B_x \approx B_z$ we can study the order of magnitude of the terms in equation (\ref{eq: 2.19}). For that we use $O$ to denominate the order of magnitude, and $T_i$ to denominate the term in the equation, with $i$ increasing from the left to the right. We start by noting that the non-magnetic solution varies typically in a scale of $H$, i.e., $O(\frac{d {\xi}_{si}}{d z})\approx H^{-1}{\xi}_{si}$. For frequencies not too far from $\omega_c$, as those seen in roAp stars, this means that $O(\frac{d {\xi}_{si}}{d z})\approx O((\omega/c) {\xi}_{si}) = O(\omega\sqrt{\rho_0/(\gamma p_0)}{\xi}_{si})$. 

Having this in mind we find that for equation (\ref{eq: 2.19}) the order of magnitude of the terms is as follows,

\begin{eqnarray}
O(T_1)\approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right), 
\end{eqnarray}

\begin{eqnarray}
O(T_2)\approx 0\left(\tilde{\beta}\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right), 
\end{eqnarray}

Due to the fact that we are in the magnetically dominated region, $\tilde{\beta}<<1$ and, consequently, $O(T_1)>>O(T_2)$. In this sense, equation (\ref{eq: 2.22}) can be written as equation (\ref{eq: 2.23}). Looking at the latter we can conclude, under the assumptions previously made, that

\begin{equation}
\label{eq: 2.23ca}
{\xi}_{\bot s} \approx O(\tilde{\beta}{\xi}_{||s}).
\end{equation}


Therefore, under the assumptions considered, we see that the component of the slow displacement perpendicular to the magnetic field is much smaller than the component of the slow displacement parallel to the magnetic field, i.e.,

\begin{equation}
{\xi}_{\bot s}<<{\xi}_{|| s}\nonumber
\end{equation}

This is in accordance with the fact that in a magnetically dominated region the slow displacement is almost acoustic and, hence, takes place essentially along the magnetic field lines.\
 

Let us now determine the order of magnitude of the terms in equation (\ref{eq: 2.24}). Also here we are considering the case of $B_x\approx B_z$. Taking into account equation (\ref{eq: 2.23ca}) we can show that $O(T_3)$ and $O(T_4)$ are as follows,

\begin{eqnarray}
O(T_3) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\xi_{||s}\right)\nonumber
\end{eqnarray}



\begin{eqnarray}
O(T_4) \approx O\left(\frac{1}{p_0}\frac{dp_0}{dz}\sqrt{\frac{\omega^2 \rho_0}{\gamma p_0}}\tilde{\beta}\xi_{|| s}\right) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\tilde{\beta}\xi_{||s}\right)\nonumber
\end{eqnarray}

Comparing $O(T_3)$ with $O(T_4)$ in equation (\ref{eq: 2.24}), we can conclude that $O(T_4)$ is always much smaller than $O(T_3)$, thus we can neglect the fourth term in comparison to the third term, and equation (\ref{eq: 2.24}) can be written as equation (\ref{eq: 2.26}).


In the order of magnitude analysis presented here we assumed that $B_x \approx B_z$. However, using the solution for $\xi_{||s}$ found and returning to equations (\ref{eq: 2.21}) and (\ref{eq: 2.22}), we can show that this solution is also appropriate in the cases of $B_x$ tending to zero and $B_z$ tending to zero. The former is equivalent to considering the case in the absence of the magnetic field, so it is necessarily in accordance with the analysis made previously. Let us now consider the case of $B_z$ tending to zero. In this case the last term on the right hand side of equation (\ref{eq: 2.29}) dominates and, therefore, $k^2_{||} \approx \frac{\omega^2\rho_0 |\bm{B}_0|^2}{\gamma p_0 B_z^2}$. Going back to the analysis of the order of magnitude, in equation (\ref{eq: 2.22}) we have,   


\begin{eqnarray}
O(T_1)\approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\frac{|\bm{B}_0|^2}{B^2_z}{\xi}_{\bot s}\right), 
\end{eqnarray}

\begin{eqnarray}
O(T_2)\approx O\left(\tilde{\beta}\frac{\omega^2 \rho_0}{\gamma p_0}{\xi}_{\bot s}\right). 
\end{eqnarray}

Thus, we can conclude, as in the previous case, that $O(T_1)$ is always much larger than $O(T_2)$, leading back to equation(\ref{eq: 2.23}).

Moreover, looking at equation (\ref{eq: 2.23}) we can conclude that in this case,

\begin{equation}
\label{eq: 2.23c}
{\xi}_{\bot s} \approx O\left(\tilde{\beta}\frac{B_x B_z}{|\bm{B}_0|^2}{\xi}_{||s}\right)
\end{equation}


Therefore, we find, as before,

\begin{equation}
{\xi}_{\bot s}<<{\xi}_{|| s}\nonumber.
\end{equation}


Let us now compare $O(T_3)$ with $O(T_4)$ in equation (\ref{eq: 2.24}) when $B_z$ tends to zero,


\begin{eqnarray}
O(T_3) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\frac{|\bm{B}_0|^2}{B^2_z}\xi_{||s}\right)\nonumber
\end{eqnarray}



\begin{eqnarray}
O(T_4) \approx O\left(\frac{\omega^2 \rho_0}{\gamma p_0}\tilde{\beta}\frac{B_x^2}{|B_0|^2}\xi_{||s}\right)\nonumber, 
\end{eqnarray}

therefore, also in this case, $O(T_3)$ is larger than $O(T_4)$, and we can neglect the fourth term in equation (\ref{eq: 2.24}), which leads us back to equation (\ref{eq: 2.26}).
So, we may conclude that the approximate solution expressed by equation (\ref{eq: 2.30c}), derived when considering $B_x \approx B_z$, is in fact an approximate solution for $\xi_{||s}$ in the more general case, since the terms of equations (\ref{eq: 2.21}) - (\ref{eq: 2.22}) that were neglected in the first case remain small, for this solution, when the condition $B_x \approx B_z$ is no longer satisfied. 

\vspace{0.3cm}

\underline{\textbf{Fast Magnetic Component}}

\vspace{0.3cm}

Similarly to what we have done for the slow acoustic component of the displacement we also study the order of magnitude of each term in the equation (\ref{eq: 2.33}). For that we shall keep in mind the condition $({\bar{\xi}}_{si})^{-1} d{\bar{\xi}}_{si}/dz >> ({\bar{\xi}}_{fi})^{-1} d{\bar{\xi}}_{fi}/dz$ assumed previously. Since $O(({\bar{\xi}}_{si})^{-1} d{\bar{\xi}}_{si}/dz) \approx O(\omega\sqrt(\rho_0/\gamma p_0))$, for equation (\ref{eq: 2.33}) we find

\begin{eqnarray}
O(T_1) < < O(T_5), \nonumber
\end{eqnarray}

\begin{eqnarray}
O(T_3) < < O(T_5). \nonumber
\end{eqnarray}

In this sense, equation (\ref{eq: 2.33}) can be written as equation (\ref{eq: 2.35}). In addition, comparing the terms in the latter equation we find that, in all cases, the fast component of the displacement perpendicular to the magnetic field is much larger than the fast component of the displacement parallel to the magnetic field, i.e.,

\begin{eqnarray}
\xi_{\bot f}>>\xi_{|| f}\nonumber.
\end{eqnarray}

Therefore we can say that the fast displacement is almost perpendicular to the direction of the magnetic field. This is not surprising, since in the magnetically dominated region this component of the displacement is expected to be essentially a magnetic wave, only slightly modified by the gas pressure.

